A Simple Functional Presentation and an Inductive Correctness Proof of the Horn Algorithm

We present a recursive formulation of the Horn algorithm for deciding the satisfiability of propositional clauses. The usual presentations in imperative pseudo-code are informal and not suitable for simple proofs of its main properties. By defining the algorithm as a recursive function (computing a least fixed-point), we achieve: 1) a concise, yet rigorous, formalisation; 2) a clear form of visualising executions of the algorithm, step-by-step; 3) precise results, simple to state and with clean inductive proofs.

==> eptcsdata.tex <==
\providecommand{\firstpage}{34}
\providecommand{\publicationstatus}{T. Kahsai and G. Vidal (Eds.): 5th Workshop on\\ Horn Clauses for Verification and Synthesis 2018 (HCVS'18).\\
EPTCS 278, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.278.6}{10.4204/EPTCS.278.6}}
\pdfoutput=1

